MedAttacker: Exploring Black-Box Adversarial Attacks on Risk Prediction Models in Healthcare

Deep neural networks (DNNs) have been broadly adopted in health risk prediction to provide healthcare diagnoses and treatments. To evaluate their robustness, existing research conducts adversarial attacks in the white/gray-box setting where model parameters are accessible. However, a more realistic black-box adversarial attack is ignored even though most real-world models are trained with private data and released as black-box services on the cloud. To fill this gap, we propose the first black-box adversarial attack method against health risk prediction models named MedAttacker to investigate their vulnerability. MedAttacker addresses the challenges brought by EHR data via two steps: hierarchical position selection which selects the attacked positions in a reinforcement learning (RL) framework and substitute selection which identifies substitute with a score-based principle. Particularly, by considering the temporal context inside EHRs, it initializes its RL position selection policy by using the contribution score of each visit and the saliency score of each code, which can be well integrated with the deterministic substitute selection process decided by the score changes. In experiments, MedAttacker consistently achieves the highest average success rate and even outperforms a recent white-box EHR adversarial attack technique in certain cases when attacking three advanced health risk prediction models in the black-box setting across multiple real-world datasets. In addition, based on the experiment results we include a discussion on defending EHR adversarial attacks.

==> fig/backup/introduction.tex <==
\section{Introduction}


The increasingly accumulated electronic health records (EHR) data and the unprecedented progress of deep neural networks (DNNs) technology have advanced the field of health analytics, especially the \emph{health risk prediction task}, which aims to predict future health status of patients according to their historical EHR data. Existing health risk prediction models mainly depend on leveraging DNNs to capture disease patterns and predict patients' future health status based on their health data. Due to the importance of health risk prediction in clinical decision making and medical resource planning, many health data companies such as KenSci,\footnote{\url{https://www.kensci.com/}} Lumiata,\footnote{\url{https://www.lumiata.com/}} and IQVIA\footnote{\url{https://www.iqvia.com/}} train their private models by using massive proprietary data and release them as a \textbf{black-box} service on the cloud. However, the connected EHR systems and risk prediction models are vulnerable against \textit{adversarial attacks} for a number of financial reasons.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.4\textwidth]{fig/sample.pdf} 
    \vspace{-0.15in}
    \caption{Illustration of EHR data. }
    \label{fig:data}
    \vspace{-0.15in}
\end{figure}
%due to the restrictions on sharing proprietary information (e.g., the disease model and patient data used in model training). .. However, the connected EHR systems and risk prediction models are vulnerable for \textit{adversarial attacks} for a number of financial reasons. 
%Recent years have witnessed unprecedented progress on applying deep learning techniques in different application domains such as computer vision, natural language processing (NLP), and healthcare. One of the key tasks in the healthcare domain is \textit{risk prediction}, which aims to predict future health status of patients according to their historical electronic health record (EHR) data. 
% Risk prediction is relevant to many questions in clinical medicine, public health, and epidemiology, and the predicted risks of a specific diagnosis or health outcome can be used to support decisions by patients, doctors, health policy makers, and academics.
% Thus, several commercial health companies such as KenSci\footnote{\url{https://www.kensci.com/}}, Lumiata\footnote{\url{https://www.lumiata.com/}}, and IQVIA\footnote{\url{https://www.iqvia.com/}} have their own products or systems to target this task using state-of-the-art deep learning techniques. 


Since good understanding of the vulnerability of deep risk prediction models can help  proactively prevent the high-risk attacks, researchers start to investigate the EHR adversarial attack. Existing studies mainly focus on \textbf{white/gray-box adversarial attacks}, which assume attackers can access the parameters of risk prediction models. For example, Sun \textit{et.\ al.}~\cite{sun2018identify} propose to identify susceptible locations in clinical time series data by employing a recurrent neural network (RNN) as a time-preferential minimum attack model and focus on real-valued continuous variables such as vital sign and lab measurements. An \textit{et.\ al.}~\cite{an2019longitudinal} propose LAVA that aims to generate adversarial examples to attack EHR data. 
In~\cite{wang2020attackability}, Wang \textit{et.\ al.} propose an efficient orthogonal matching pursuit-guided method for white-box evasion attack on discrete EHR data. However, the assumptions of white/gray-box settings are often invalid in real-world practice because the parameters of proprietary models are inaccessible. Thus, it is desirable to have a \textbf{black-box adversarial attack} solution for understanding the vulnerability of DNNs based risk prediction models.
% Although deep learning-based models have shown their superiority in the risk prediction task compared with traditional machine learning approaches~\cite{ma2017dipole, choi2016retain, song2017attend, luo2020hitanet,zhang2020two}, they still suffer from the vulnerability issue by \textit{adversarial attacks} as in other domains such as computer vision~\cite{goodfellow2014explaining,carlini2017towards,moosavi2016deepfool, tang2020embarrassingly,pang2020advmind,chen2020rays} and natural language processing~\cite{zang2020learning,ren2019generating,gao2018black, li2019textbugger,jia2017adversarial,garg2020bae}. 
% However, the work on investigating the vulnerability of risk prediction models is still at a very preliminary stage. As far as we know, there are only three studies working on the vulnerability of risk prediction models against \textbf{white/gray-box adversarial attacks}. Sun \textit{et.\ al.}~\cite{sun2018identify} propose to identify susceptible locations in clinical time series data using a recurrent neural network (RNN) based time-preferential minimum attack model and focus on real-valued continuous variables such as vital sign and lab measurements. An \textit{et.\ al.} propose LAVA~\cite{an2019longitudinal} that aims to generate adversarial examples to attack EHR data. 
% In~\cite{wang2020attackability}, Wang \textit{et.\ al.} propose a computationally efficient orthogonal matching pursuit-guided attack method for white-box evasion attack on discrete EHR data. 
% However, in the real-world applications, it is nearly impossible to assess all the source code of commercial risk prediction models. In other words, these approaches are too ideal to be used in practice for validating the robustness of risk prediction models. Thus, it is essential to design a \textbf{black-box adversarial attack} method for the risk prediction task to understand the vulnerability of deep learning techniques in healthcare.

\smallskip
\noindent 
\textbf{Data Challenge. \label{Sec: data challenge}}
The challenge of designing black-box adversarial attack models mainly stems from the unique structure of EHR data. As shown in Figure~\ref{fig:data}, each longitudinal EHR is a sequence of patient visits that show their evolving conditions as well as sporadic health incidences, where each visit includes many unordered medical codes. Although some draw an analogy between EHR models and natural language processing (NLP) models by considering the diagnosis codes as words and the whole record as a document, the text adversarial attack models~\cite{zang2020learning,ren2019generating,gao2018black, li2019textbugger} cannot be directly applied to the EHR modeling due to the unique EHR structure, especially the \textbf{unordered} codes within each visit and the \textbf{incidental} nature of many hospital visits. That being said, unlike  NLP models, for EHR models there can be no explicitly relations among codes within a visit, or among two consecutive visits.
%The challenge of designing such a black-box adversarial attack model mainly stems from the uniqueness of EHR data, which consist of longitudinal patient visits as shown in Figure~\ref{fig:data}. Intuitively, each visit can be considered as a sentence, and the whole EHR data are treated as a document. In such a way, text-based adversarial attack models~\cite{zang2020learning,ren2019generating,gao2018black, li2019textbugger} can be directly applied to the risk prediction task. However, this naive conversion ignores the unique characteristics of EHR data. In fact, patient visits are different from sentences. Each sentence consists of several words, and there exist syntactic relations between two consecutive words. However, \textit{each patient visit contains several discrete yet unordered medical codes} such as ICD codes\footnote{\url{https://www.who.int/standards/classifications/classification-of-diseases}}, and there is no explicitly relations among them. Besides, two consecutive sentences have more or less semantic relations. However, \textit{the principle diagnoses of two successive visits may be totally different}. Thus, these unique characteristics makes black-box adversarial attacks on risk prediction models in healthcare more challenging.


\smallskip
\noindent 
\textbf{Technical Challenge.} 
% Although EHR data are different from text data, they still share some similar patterns. Thus, text-based black-box adversarial attack methods are important references to risk prediction attacks.  
Existing black-box techniques attacking discrete data like text usually  firstly find  sensitive words, and then select candidate words to replace the sensitive ones. These two steps are implemented by either score-based methods that are designed to quantify the sensitivity level of each word~\cite{ren2019generating,gao2018black, li2019textbugger} or reinforcement learning ones~\cite{zang2020learning} that aim at learning an optimal policy under which a series of substitution operations are interactively conducted to generate adversarial examples. Despite their good performance,  they either only focus on the importance of a single word, or may only work when the number of words is limited and the  substitute space is small. 

As Figure~\ref{fig:data} shows, for EHR data, the number of visit for each patient is not too large, and within each visit the number of ICD codes\footnote{\url{https://www.cdc.gov/nchs/icd/icd9cm.htm}} is also limited. These characteristics seem to fit the application of reinforcement learning-based models. However, the number of substitutes of a specific code may be huge according to the Clinical Classification Software,\footnote{\url{https://www.hcup-us.ahrq.gov/toolssoftware/ccs/AppendixASingleDX.txt}} which can lead to the failure of reinforcement learning-based models. On the contrary, score-based approaches can directly replace words based on the calculated saliency scores without dynamically searching the whole candidate space, which avoids the shortage of reinforcement learning-based approaches. Thus, it raises a question: \textit{Is it possible to ``hybridize'' those two kinds of methods for solving our problem?}

\smallskip
\noindent 
\textbf{Our Approach.} 
To solve the aforementioned challenges, in this paper, we propose a new black-box adversarial attack method named~{\name} to explore the vulnerability of health risk prediction models. To address the challenges brought by the unique EHR structure, {\name} takes a hybrid approach that bridges score-based and reinforcement learning attack models. {\name} has two steps: \textbf{hierarchical position selection} and  \textbf{substitute selection}. To be specific, the first step of~{\name} is to calculate the contribution score of \textit{each visit} by taking the context into consideration. Next, it calculates the saliency score of \textit{each ICD code} within each visit. Using the contribution scores and saliency scores as the initialized policy parameters, {\name} adopts a reinforcement learning framework to select the attacked positions in the EHR to avoid the greedy scored-based mechanism that may not lead to generating globally optimized adversarial samples. Finally, after determining the attacked positions, {\name} selects the substitute code for the original one by the score change it can bring, and the selected substitute is the one that can bring the highest score change.


\smallskip
\noindent 
\textbf{Contributions.}
To sum up, our contributions are as follows:
\begin{itemize}[leftmargin=*]
    \item To the best of our knowledge, we are the first to explore the vulnerability of health risk prediction models via black-box adversarial attacks. Compared with  white/gray-box setting, black-box adversarial attack is  more realistic, so our work can better expose the vulnerability of risk prediction models in the real world.
    \item We propose a new black-box adversarial attack method called~{\name}, which is motivated to solve the challenges brought by the unique EHR data structure and fully leveraging the advantages of score-based and reinforcement learning approaches. {\name} attacks the risk prediction models by taking the temporal context into consideration, and it is better at approximating globally optimized adversarial samples by adopting a reinforcement learning framework.
    % \item The experimental results show that {\name} can generate more adversarial examples to fool three representative risk prediction models on three real-world healthcare datasets compared with state-of-the-art black-box attack models, and it even performs better than white-box model LAVA~\cite{an2019longitudinal} on the Dementia dataset. In addition, we include a discussion on the defense against adversarial attacks for risk prediction models.
    \item We compare {\name} against several state-of-the-art black-box attack methods in terms of attack success rate across  three real-world healthcare datasets. Results show that {\name} can generate more adversarial examples on average, and even performs better than white-box model LAVA~\cite{an2019longitudinal} in the Dementia dataset. Lastly, we include a discussion on the defense against adversarial attacks for risk prediction models.
\end{itemize}


% \section{Introduction}
% Recent years have seen great progress in the application of deep neural networks (DNNs) in the healthcare risk prediction problem. Risk prediction~\cite{ma2017dipole, choi2016retain, song2017attend, luo2020hitanet} is a binary classification task that requires machine learning models to make future predictions on the status of patients with their electronic health records (EHRs) as inputs. Among the various kinds of EHR, one of the most widely used form of EHRs is encoded by a high dimensional symptom dictionary such as the International Classification of Diseases (ICD)~\footnote{\url{https://www.who.int/standards/classifications/classification-of-diseases}} system, which is the EHR data that we are focused on in this paper. When the EHRs of patients are recorded by the ICD codes, their symptoms in each visit will be recorded by individual unique codes. Such a property of the ICD-based EHR makes the risk problem  similar to the text classification problem in the natural language processing (NLP) domain, where the whole EHR of a patient can be regarded as a document and each visit encoded by ICD codes can be regarded as a sentence. 

% The data mining community has shown huge interest on the vulnerability of DNNs against adversarial attacks in the general domains such as images~\cite{goodfellow2014explaining,carlini2017towards,moosavi2016deepfool} and texts~\cite{zang2020learning,ren2019generating,gao2018black, li2019textbugger} recently. Speaking of adversarial attacks, it is a technique of generating adversarial samples from the original inputs to fool the target DNNs and cause them to make mistakes, which is essential in investigating the safety of machine learning models. The vulnerability of risk prediction DNNs are also worth exploring considering the sensitivity of medical data. However, the work on investigating the vulnerability of risk prediction DNNs is still in the early stage. There is few work on the vulnerability of risk prediction DNNs against adversarial attack, especially the black-box ones, and the current representative work on attacking risk prediction models includes~\cite{an2019longitudinal} and~\cite{sun2018identify}.~\cite{sun2018identify} mainly focuses on attacking healthcare predictive models applied in EHRs described by continuous variables from vital sign measurements and lab events, while \cite{an2019longitudinal} is about white-box and grey-box adversarial attacks on ICD-based EHR. Considering the real-world situation in the healthcare domain, there is still a challenge of designing a black-box adversarial attack method for risk prediction method to understand the vulnerability of DNNs, which is a more difficult and realistic setting because it does not allow the adversarial attack methods to use the gradients of risk prediction models.

% In this paper, we are focused on designing a black-box adversarial attack method which can help explore the vulnerability of risk prediction DNNs in the healthcare domain. Although risk prediction task can be regarded as a special text classification task and existing black-box adversarial attack methods in the NLP domain can be used in our case, the direct adoption is not optimal for attacking risk prediction models for they mostly ignore the temporal correlation between the visits of the same patient, which are the important information used in risk prediction. Thus, we propose a new black-box adversarial attack method termed as~{\name}. To be specific, the first step of~{\name} is calculating the contribution score of each visit by taking the context into consideration. Next, it calculates the saliency score of each ICD code. After getting the contribution scores and saliency scores,~{\name} follows a reinforcement learning framework to select the positions to be attacked in the EHR to avoid the greedy mechanism that may not lead to generating globally optimized adversarial samples. Finally, after determining the positions to be attacked,~{\name} selects the substitution codes by the changes they bring to generate the adversarial samples.

% To sum up, our contributions are as follows:
% \begin{itemize}
%     \item To the best of our knowledge, we are the first to explore the design of black-box adversarial attack method to explore the the vulnerability of risk prediction DNNs in the healthcare domain. Our method takes a more realistic scenario, i.e, the black-box setting, into consideration, which is helpful in evaluating the vulnerability of risk prediction DNNs.
%     \item We propose a new adversarial attack method called~{\name} which is more suitable in dealing with EHR data.~{\name} attacks the risk prediction DNNs by taking the temporal context into consideration, and it is better at approximating globally optimized adversarial samples by adopting an reinforcement learning framework.
%     \item The experimental results show that~{\name} can generate more adversarial examples to fool representative risk prediction models. In addition, we include a discussion on the defense of adversarial attacks for risk prediction DNNs.
% \end{itemize}






